Tackling the muon identification in water Cherenkov detectors problem for the future Southern Wide-field Gamma-ray Observatory by means of Machine Learning

This paper presents several approaches to deal with the problem of identifying muons in a water Cherenkov detector with a reduced water volume and 4 PMTs. Different perspectives of information representation are used and new features are engineered using the specific domain knowledge. As results show, these new features, in combination with the convolutional layers, are able to achieve a good performance avoiding overfitting and being able to generalise properly for the test set. The results also prove that the combination of state-of-the-art Machine Learning analysis techniques and water Cherenkov detectors with low water depth can be used to efficiently identify muons, which may lead to huge investment savings due to the reduction of the amount of water needed at high altitudes. This achievement can be used in further research to be able to discriminate between gamma and hadron induced showers using muons as discriminant.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 1342 2019-01-29 17:20:57Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard *.sty *.bib figs/*) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := /bin/bash
PDFS := $(addsuffix .pdf, $(TARGETS))

ifeq (, $(shell which latexmk))
  LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)
  # 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
  COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'
  define basic_latex_rule
    for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
  endef
  ifeq ($(USEBIBTEX), 1)
    define latex_rule
      $(LATEX) $< ; bibtex $*
      $(call basic_latex_rule)
    endef
  else
    define latex_rule
      $(call basic_latex_rule)
    endef
  endif
else
  define latex_rule
    latexmk $(if $(filter 1, $(USEPDFLATEX)), -pdf, ) $<
  endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,.maf,.fff,.lot,.ttt,.bcf,.run.xml,.fdb_latexmk,.fls,.synctex.gz}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

